Diffusion Models for Counterfactual Explanations

Counterfactual explanations have shown promising results as a post-hoc framework to make image classifiers more explainable. In this paper, we propose DiME, a method allowing the generation of counterfactual images using the recent diffusion models. By leveraging the guided generative diffusion process, our proposed methodology shows how to use the gradients of the target classifier to generate counterfactual explanations of input instances. Further, we analyze current approaches to evaluate spurious correlations and extend the evaluation measurements by proposing a new metric: Correlation Difference. Our experimental validations show that the proposed algorithm surpasses previous State-of-the-Art results on 5 out of 6 metrics on CelebA.

==> sections/001introduction.tex <==
\section{Introduction}

Convolutional neural networks (CNNs) reached performances unimaginable a few decades ago, thanks to the adoption of very large and deep models (e.g. with hundreds of layers and nearly billions of trainable parameters). Yet, it is difficult to explain their decisions because they are highly non-linear and over-parametrized. Moreover, for real-life applications, if a model exploits spurious correlations of data to forecast a prediction, the end-user will doubt the validity of the decision. Particularly, in high-stake scenarios like medicine or critical systems, ML must guarantee the usage of correct features to compute a prediction and prevent counterfeit associations. For this reason, the Explainable Artificial Intelligence (XAI) research field has been growing in recent years to progress towards understanding the decision-making mechanisms in black-box models. 

In this paper, we focus on \emph{post-hoc} explanation methods. Notably, we concentrate on the growing branch of Counterfactual Explanations (CE)~\cite{wachter2018CounterfactualExplanationsOpening}. CEs aim to create minimal but meaningful perturbations of an input sample to change the original decision given by a black-box model. 
Although the objective between CE and adversarial examples share some similarities~\cite{pawelczykExploringCounterfactualExplanations2021}, the CEs' perturbations must be understandable. In contrast, adversarial examples~\cite{madry2018towards} contain high-frequency noise \textit{indistinguishable} for the human eye.
On overall, CEs target three goals: \textit{(i)} create proximal images with sparse modifications, \textit{i.e.} instances with the smallest perturbation, \textit{(ii)} the explanations must be realistic and understandable by a human, and \textit{(iii)} the counterfactual generation method must create diverse instances. In general, counterfactual explanations seek to reveal the learned correlations related to the model's decisions.

Multiple works on CE use generative models to create tangible changes in the image~\cite{sauer2021counterfactual,Rodriguez_2021_ICCV,Joshi2018xGEMsGE}. Further, these architectures recognize the factors to generate images near the image-manifold~\cite{arora2018do}. Given the recent advances within image synthesis community, we propose DiME: \underline{Di}ffusion \underline{M}odels for counterfactual \underline{E}xplanations. DiME harnesses the denoising diffusion probabilistic models~\cite{NEURIPS2020_4c5bcfec} to produce CEs. For simplicity, we will refer to these models as diffusion models or DDPMs. To the best of our knowledge, we are the first to exploit these new synthesis methods in the context of CE. 

Diffusion models offer several advantages compared to alternate generative models, such as GANs. First of all, DDPMs have several latent spaces; each one controls coarse and fine-grained details. We take advantage of low-level noise latent spaces to generate semantically-meaningfully changes in the input image. These spaces only have been recently studied by~\cite{meng2022sdedit} for inpainting. Secondly, due to their probabilistic nature, they produce a diverse set of images. Stochasticity is ideal for CEs because multiple explanations may explain a classifier's error modes. Third, Nichol and Dhariwal~\cite{nichol2021improved} results suggest that DDPMs cover a broader range of the target image distribution. Indeed, they noticed that for similar FID, the recall is much higher on the improved precision-recall metrics~\cite{Kynkaanniemi2019}. Finally, DDPMs' training is more stable than the State-of-the-Art synthesis models, notably GANs. Due to their relatively new development, DDPMs are under-studied, and multiple aspects are yet to be deciphered. 

We contribute a small step into the XAI community by studying the low-level noised latent spaces of DDPMs in the context of counterfactual explanations. We summarize our contributions as follows:
\begin{itemize}
    \item DiME uses the recent diffusion models to generate counterfactual examples. Unlike other generative models, our CE algorithm does not require training the diffusion model in a conditioned way or retraining it using gradients, \emph{i.e.} we rely on a single trained unconditional DDPM to achieve our objective.
    \item We derive a new way to leverage an existing (target) classifier to guide the generation process instead of ones trained on noisy instances. 
    \item We set a new State-of-the-Art result on CelebA, surpassing the previous works on counterfactual explanations on the FID, FVA, and MNAC metrics for the \textit{Smile} attribute and the FID and MNAC for the \textit{Young} feature.
    \item We show that the MNAC provides a false sense of evaluating counterfactuals correctly. So we introduce a new metric, dubbed Correlation Difference, to evaluate subtle spurious correlations on a CE setting.
\end{itemize}

To further boost research on counterfactual explanations, we will make our code and models publicly available upon publication. 


==> sections/003methodology_loic.tex <==
\section{Methodology}

\subsection{Preliminaries}

We begin by introducing the generation process of diffusion models. They rely on two Markov chain sampling schemes that are inverse of one another. In the forward direction, the sampling starts from a natural image $x$ and iteratively sample $z_1,\cdots,z_T$ by replacing part of the signal with white Gaussian noise. More precisely, letting $\beta_t$ be a prescribed variance, the forward process follows the recursive expression:
\begin{equation} \label{eq:degradation_onestep}
    z_t \sim \mathcal{N} (\sqrt{1-\beta_t}\,z_{t-1},  \beta_t \,I),
\end{equation}
where $\mathcal{N}$ is the normal distribution, $I$ the identity matrix, and $z_0 = x$. In fact, this process can be simulated directly from the original sample with 
\begin{equation} \label{eq:degradation}
    z_t \sim \mathcal{N} (\sqrt{\alpha_t}x, (1 - \alpha_t) I),
\end{equation}
where $\alpha_t := \prod_{k=1}^t (1 - \beta_k)$. For clarification, through the rest of the paper, we will refer to clean images with an $x$, while noisy ones with a $z$. 


In the reverse process, a neural network recurrently denoises $z_T$ to recover the previous samples $z_{T-1},\cdots, z_0$. This network takes the current time step $t$ and a noisy sample $z_t$ as inputs, and produces an average sample $\mu(t, z_t)$ and a covariance matrix $\Sigma(t,z_t)$, shorthanded as $\mu(z_t)$ and $\Sigma(z_t)$, respectively. Then $z_{t-1}$ is sampled with 
\begin{equation} \label{eq:sampling}
    z_{t-1} \sim \mathcal{N}(\mu(z_t), \Sigma(z_t)).
\end{equation}
So, the DDPM algorithm iteratively employs Eq.~\ref{eq:sampling} to generate an image $z_0$ with zero variance, \textit{i.e.} a clean image. Some diffusion models use external information, such as labels, to condition the denoising process. However, in this paper, we employ an unconditional DDPM. 

In practice, the series of variances $\{\beta_t\}$ are chosen such that $z_T\sim \mathcal{N}(0,I)$. Further, the DDPM's trainable parameters are fitted so that the reverse and forward processes share the same distribution. For details on training schemes, we recommend the studies of Ho \emph{et al.}~\cite{NEURIPS2020_4c5bcfec} and Nichol and Dhariwal~\cite{nichol2021improved} to the reader. Once the network is trained, one can rely on the reverse Markov chain process to generate a clean image from a random noise image $z_T$. Besides, the sampling procedure can be adapted to optimize some properties following the so-called \emph{guided diffusion} scheme proposed in \cite{Dhariwal2021DiffusionMB}\footnote{In \cite{Dhariwal2021DiffusionMB}, the guided diffusion is restricted to a specific classification loss. Still, for the sake of generality and conciseness, we provide its extension to an arbitrary loss}:
\begin{equation} \label{eq:generalized-diff}
    z_{t-1} \sim \mathcal{N}(\mu(z_t) - \Sigma(z_t)\, \nabla_{z_t} L(z_t; y), \Sigma(z_t)),
\end{equation}
where $L$ is a loss function using $z_t$ to specify the wanted property of the generated image, for example, to condition the generation on a prescribed label $y$.

\subsection{DiME: Diffusion Models for Counterfactual Explanations}

We take an image editing standpoint on CE generation, as illustrated Fig.~\ref{fig:baselinecf}. We start from a query image $x$. Initially, we rely on the forward process starting from $x_\tau=x$ to compute a noisy version $z_\tau$, with $1\leq\tau\leq T$. Then we go back in the reverse Markov chain using the guided diffusion (Eq~\ref{eq:generalized-diff}) to recover a counterfactual (hence altered) version of the query sample. Building upon previous approaches for CEs based on other generative models~\cite{Singla2020Explanation,wachter2018CounterfactualExplanationsOpening,jacob2021steex}, we rely on a loss function composed of two components to steer the diffusion process: a classification loss $L_{class}$, and a perceptual loss $L_{perc}$. The former guides the image edition into imposing the target label, and the latter drives the optimization in terms of proximity.

\input{figures/main-figure}

In the original implementation of the guided diffusion~\cite{Dhariwal2021DiffusionMB}, the loss function uses a classifier applied directly to the current noisy image $z_t$. This approach is appropriate since the considered classifier can make robust predictions under noisy observations, \textit{i.e.} it was trained on noisy images. Regardless, such an assumption on the classifier under scrutiny would imply a substantial limitation in the context of counterfactual examples.
We circumvent this obstacle by adapting the guided diffusion mechanism. To simplify the notations, let $x_t$ be the clean image produced by the iterative unconditional generation on Eq~\ref{eq:sampling} using as the initial condition $z_t$. In fact, this makes $x_t$ a \textit{function} of $z_t$ because we denoise $z_t$ recursively with the diffusion model $t$ times to obtain $x_t$. 
Luckily, we can safely apply the classifier to $x_t$ since it is not noisy. So, we express our loss as:
\begin{equation}\label{eq:loss-func}
    L(z_t;y, x) = \mathbb{E}\left[ \lambda_{c} L_{class}(C(y|x_t)) + \lambda_{p} L_{perc}(x_t, x)\right]:=\mathbb{E}\left[\tilde L(x_t; y, x)\right],
\end{equation}
where $C(y|x_t)$ is the posterior probability of the category $y$ given $x_t$, and $\lambda_c$ and $\lambda_p$ are constants.
Note that an expectation is present due to the stochastic nature of $x_t$. In practice, computing the loss gradient would require sampling several realizations of $x_t$ and taking an empirical average. We restrict ourselves to a single realization per step $t$ for computational reasons and argue that this is not an issue. Indeed, we can partly count on an averaging effect along the time steps to cope with the lack of individual empirical averaging. Besides, the stochastic nature of our implementation is, in fact, an advantage because it introduces more diversity in the produced CEs, a desirable feature as advocated by \cite{Rodriguez_2021_ICCV}.

Using this strategy, the dependence of the loss on $x_t$, rather than directly from $z_t$, renders the gradient computation more challenging.
Indeed, formally it would require to apply back-propagation from $x_t$ back to $z_t$: 
\begin{equation}\label{eq:clean-grads-general}
    \nabla_{z_t}L(z_t; y, x) = \left(\frac{Dx_t}{Dz_t}\right)^T\cdot\nabla_{x_t}\tilde L(x_t; y, x).
\end{equation}
Unfortunately, this computation requires retaining Jacobian information throughout the entire computation graph, which is very deep when $t$ is close to $\tau$. As a result, backpropagation is too memory intensive to be considered an option. To bypass this pitfall, we shall rely on the forward sampling process, which operates in a single stage (Eq.~\ref{eq:degradation}). Using the reparametrization trick~\cite{Kingma2014}, one obtains
\begin{equation}
    z_t = \sqrt{\alpha_t} x_t + \sqrt{1 - \alpha_t} \epsilon, \; \epsilon \sim \mathcal{N}(0, \mathbf{I}).
\end{equation}
Thus, by solving $x_t$ from $z_t$, we can leverage the gradients of the loss function with respect to the noisy input, a consequence of the chain rule. Henceforth, the gradients of $L$ with respect to the noisy image become
\begin{equation} \label{eq:clean-grads}
    \nabla_{z_t}L(z_t; y, x) = \frac{1}{\sqrt{\alpha_t}} \nabla_{x_t}\tilde L(x_t; y, x).
\end{equation}
This approximation is possible since the DDPM estimates the reverse Markov chain to fit the forward corruption process. Thereby, both processes are similar.

To sum up, Fig.~\ref{fig:baselinecf} depicts the generation of a counterfactual explanation with our algorithm: DiME. We start by corrupting the input instance $x=x_\tau$ following Eq.~\ref{eq:degradation} up to the noise level $t=\tau$. Then, we iterate the following two stages until $t=0$: \textit{(i)} First, using the gradients of the previous clean instance $x_{t-1}$, we guide the diffusion process to obtain $z_{t-1}$ using Eq.~\ref{eq:generalized-diff} with the gradients computed in Eq.~\ref{eq:clean-grads}. \textit{(ii)} Next, we estimate the clean image $x_t$ for the current time step $z_{t-1}$ with the unconditional generation pipeline of DDPMs. The final instance is the counterfactual explanation. If we do not find an explanation that fools the classifier under observation, we increase the constant $\lambda_c$ and repeat the process.

\textbf{Implementation Details.} 
To train the unconditional DDPM model, we used the publicly available code of~\cite{Dhariwal2021DiffusionMB}. We include all training and architectural details in the supplemental material. In practice, we incorporate additionally an $\ell_1$ loss, $\eta || z_t - x ||_1$, between the noisy image $z_t$ and the input $x$ to improve the $\ell_1$ metric on the pixel space. We empirically set $\eta$ small to avoid any significant impact on the quality of the explanations. Our diffusion model generates faces using 500 diffusion steps from the normal distribution. We re-spaced the sampling process to boost inference speed to generate images with 200 time-steps at test time. We use the following hyper-parameters settings:  $\lambda_{p}=30$, $\eta=0.05$, and $\tau=60$. Finally, we set $\lambda_{c} \in \{8, 10, 15\}$ to iteratively find the counterfactuals. We consider that our method failed if we do not find any explanation after exhausting the values of $\lambda_c$.

==> sections/temp_exp.tex <==

\section{Experiments}

\textbf{Experimental Setup.} 
In this section, we evaluate our CE approach using standard metrics. Also, we develop new tools to go beyond the current evaluation practices.
Let us then recap the principles of current evaluation metrics, following previous works~\cite{Rodriguez_2021_ICCV,Singla2020Explanation}. 
The first goal of CEs is to create {\em realistic} explanations that {\em mislead} the classifier under observation.
The capacity to fool the classifier is typically exposed as a flip ratio (FR). 
Following the image synthesis research literature, the Frechet Inception Distance~\cite{NIPS2017_8a1d6947} (FID) measures the fidelity of the image distribution. 
The second goal of CE methods is to create proximal and sparse images.
Among other tools, the XAI community adopted the Face Verification Accuracy~\cite{8373813} (FVA) and Mean Number of Attributes Changed (MNAC)~\cite{Rodriguez_2021_ICCV}.
On the one hand, the MNAC metric looks at the face attributes that changed between the input image and its counterfactual explanation, disregarding if the individual's identity changed. 
On the other hand, the FVA looks at the individual's identity without considering the difference of attributes. 

Despite their usefulness, the previous metrics miss two important properties of CEs.
Indeed, following \cite{Rodriguez_2021_ICCV}, to give a sense of trust in a classifier, the CEs must also produce diverse explanations and ensure that the classifier is not subject to spurious correlations.
On the one hand, generating diverse explanations is useful to discover the brittleness of CNNs. 
Mothilal, R. \textit{et al.}~\cite{Mothilal2020ExplainingML} propose a pair-wise distance to evaluate the diversity of counterfactual examples. 
Nevertheless, this work is exclusively dedicated to tabular data. 
We propose a simple adaptation to images based on the LPIPS metric \cite{Zhang_2018_CVPR_Unreasonable}. 

On the other hand, current assessments to detect spurious correlations (e.g. in \cite{Singla2020Explanation}) are quite extreme.
They rely on modified datasets by entangling two attributes artificially to a full extent, e.g. all male are smiling and all women are not. 
They also assume that in standard benchmarks, attributes are not entangled at all. 
Under this assumption, a classifier trained in this settings can be safely used as an oracle for the attributes, as proposed for computing MNAC. 
%We actually show in Figure~\ref{fig:correlation} that this assumption can be largely erroneous and therefore challenge the validity of the derived metrics.
We actually show that this assumption can be largely erroneous and therefore challenge the validity of the derived metrics.
Based on our analysis, we designed a metric called {\em Correlation Difference} to assess if subtle ``spurious correlations'' are adequately exposed by a counterfactual approach.


\textbf{Dataset.} 
In this paper, we study the CelebA dataset~\cite{liu2015faceattributes}. Following standard practices, we preprocess all images to a $128\times128$ resolution.
CelebA contains 200k images, labeled with 40 binary attributes.
Previous works validate their methods on the \emph{smile} and \emph{young} binary attributes, ignoring all other features. 
Finally, the architecture to explain is a DenseNet121~\cite{Huang_2017_CVPR}.
Given the binary nature of the task, the target label is always the opposite of the prediction. 
If the model correctly estimates an instance's label, we flip the model's forecast. 
Else, we modify the input image to classify the image correctly. 

\subsection{Realism, Proximity and Sparsity Evaluation} \label{sec:quant-val}

\input{tables/main-results}


To compute the FID, the FVA, and the MNAC, we consider only those successful counterfactual examples, following previous studies~\cite{Rodriguez_2021_ICCV,Singla2020Explanation}.
% To compute the FVA, we used the cosine similarity between the input image and its produced counterfactual on the feature space of a ResNet50~\cite{He2016DeepRL} pretrained model on VGGFace2~\cite{8373813}.
The FVA is the standard metric for face recognition. 
To measure this value, we used the cosine similarity between the input image and its produced counterfactual on the feature space of a ResNet50~\cite{He2016DeepRL} pretrained model on VGGFace2~\cite{8373813}.
The instance and the explanation share the same identity if the similarity is higher than 0.5.
So, the FVA is mean number of faces and their corresponding CE with the same identity.
To compute the MNAC, we fine-tuned the VGGFace2 model on the CelebA dataset.
We refer to the fine-tuned model as the \emph{oracle}.
Thus, the MNAC is the mean number of the changed attributes.
For a fair comparison with previous State-of-the-Art, we trained all classifiers, including the fine-tuned ResNet50 for the MNAC assessment, using the DiVE's~\cite{Rodriguez_2021_ICCV} available code.

DiVE do not report their success rate. 
This rises the concern of the fairness to compare our methods. 
Since the metrics are highly dependant on the number of samples, especially the FID, we recomputed their CEs. 
To our surprise, their flip ratio was quite low (44.6$\%$ for the smile category). 
In contrast, we achieved a success rate of 97.6 and 98.9 for the smile and young attributes, respectively.
Therefore, we calculate the counterfactual explanations with 100 optimization steps and reported the results as DiVE$^{100}$. 
DiVE$^{100}$'s success rates are $92.0\%$ for smile and $93.4\%$ for young, which is comparable to ours. 

We show DiME's performance in Table~\ref{tab:main_results}. 
Our method beats the previous literature in five out of six metrics. 
For instance, we have a $\sim$10 fold improvement on the FID metric for the smile category, while the young attribute has an $\sim$8 fold improvement. 
We credit these gains to the generative capabilities of the diffusion model. 
Further, our generation process does not require entirely corrupting the input instance; hence the coarse details of the image remain. 
The other methods use latent space-based architectures. 
Thus, they require to compact essential information removing outlier data. 
Consequently, the generated CEs cannot reconstruct the missing information, losing significant components of the image statistics. 
Regarding DiVE$^{100}$ results, the over-optimization clearly destroys most aspects that make a person's identity and its attributes. 


Regarding the smile category, the input's gradients are centralized due to the local characteristics of the attribute. 
So, the gradients do not corrupt essential regions in the guided denoising process, enabling our model to perform better in the FVA metric. 
For the other methods, small changes in the image require significant modifications due to the bottleneck. 
In contrast, editing notable features for the face is harder for our model. 
The young feature must change the general appearance of the face. 
Hence, the gradients of the classifier are not sparse. 
Therefore, the gradients might steer the diffusion process in an unwanted direction. 
As a result, small essential details change, resulting in a identity swap.

\subsection{Diversity Assessment}

One of the most crucial traits of counterfactual explanations methodologies is the ability to create multiple and diverse examples~\cite{Rodriguez_2021_ICCV,Mothilal2020ExplainingML}. 
As stated in the methodology section, DiME's stochastic properties enable the sampling of diverse counterfactuals. 
To measure the capabilities of different algorithms to produce multiple explanations, we computed the mean pair-wise LPIPS~\cite{Zhang_2018_CVPR_Unreasonable} metric between five independent runs. 
A higher LPIPS means increased perceptual dissimilarities between the explanations, hence, more diversity. 
To compute the evaluation metric we use all counterfactual examples, even the unsuccessful instances, because we search the capacity of exploring different traits. 
Note that, we exclude the input instance to compute the metric since we search for the dissimilarities between the counterfactuals. 
We evaluate DiME's performance with DiVE$^{100}$ and its Fisher Spectral variant on a small partition of the validation subset; more information on section~\ref{sec:ablations}.
% Both versions produce eight counterfactual explanations simultaneously and have an explicit mechanism to create different images. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.83\textwidth]{images/diversity.pdf}
    \caption{\textbf{Diversity Counterfactual examples.} The classifier predicts first two input images as non-smiley and the last two as smiley. Our CE pipeline is capable of synthesising diverss counterfactuals without any explicit mechanism.}
    \label{fig:diversity}
\end{figure}

% Our experimentation with DiVE shows that their success rate is relatively low. 
% Hence, we set their optimization iterations to 100 to reach a similar FR. 
% Even with this fine-tuned hyperparameter, DiVE Fisher Spectral's FR is substantially worst and does not achieve comparable success rates. 
We visualize some examples in Fig.~\ref{fig:diversity} and show the performance of the five runs on the supplementary material. 
We obtained an LPIPS value of 0.213. 
In contrast, DiVE~\cite{Rodriguez_2021_ICCV} and its Spectral Fisher variant obtained an LPIPS of 0.044 and 0.086, respectively. 
Recall that DiME does not have an explicit mechanism to create diverse counterfactuals. 
Its only mechanism is the stochasticity within the sampling process, refer to Eqs.~\ref{eq:sampling} and~\ref{eq:generalized-diff}.
In contrast, DiVE has a diversity loss when optimizing the eight explanations. 
Yet, our methodology achieves higher diversity with the LPIPS metric even without an explicit mechanism.


\subsection{Discovering Spurious Correlations}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/cd-top10.pdf}
    \caption{\textbf{Spurious Correlation Detection.} We show the top 9 most correlated attributes in the label space with ``smile''. We obtained the Pearson Correlation Coefficient from the ground truth on the training set. Albeit the difference in the MNAC performance, DiME and DiVE achieve to detect the spurious correlations similarly. We show all the missing attributes in the supplementary material.}
    \label{fig:correlation}
\end{figure}

The end goal of counterfactual examples is to uncover the modes of error of a target model. 
Current evaluation protocols~\cite{Singla2020Explanation} search to assess the spurious correlations by inducing artificially entanglements with two uncorrelated attributes. Conventionally, the labels of choice are smile and gender. 
So, the CE algorithm detects the spurious correlation if the target (and entangled) attribute changes both entangled traits. 
Yet simple to evaluate, a problem arises. 
This extreme evaluation assumes an uncorrelated label space, which is untrue for the vast majority of datasets. 
%entanglement does not account for the subtle relationships present in the dataset.

In fact, the CelebA dataset presents a high correlation in the label space, as seen on Fig.~\ref{fig:correlation}. 
Even the selected attributes present a considerable level of correlation. 
This phenomenon raises the concern of the value of the MNAC metric. 
As a matter of fact, optimizing the MNAC metric and detecting spurious correlation have a significant conflict. 
%Since the MNAC minimizes the number of attributes, the least number of traits must change, hiding possible spurious correlations. Therefore, we propose a new metric to evaluate the 
As stated in the literature~\cite{Rodriguez_2021_ICCV,Singla2020Explanation,wachter2018CounterfactualExplanationsOpening}, one of the most important aspects of counterfactual explanations is the capacity of creating sparse modifications. 
%Therefore, the MNAC was proposed to assess these alterations. 
%So, we argue that the MNAC conflicts with the spurious correlation detection goal of CEs. 
Nevertheless, consider the next example scenario: take two CE algorithms; the first one exposes all spurious correlations correctly. 
The second one is capable of editing the main feature solely. 
Since the first method produces many changes, we expect to have a high MNAC while the other has a low MNAC value. 
This false sense of high performance does not reflect the true accomplishment of the first model: detecting spurious correlations.
So, we extend the MNAC measurement and propose the Correlation Difference (CD) metric to assess the spurious correlation detection correctly. 

The goal of CD is to measure the difference between the true correlations and the changes produced by the explanations. 
To achieve this, let $c_{qa}$ be the true correlation computed on the label space between the attribute labels $q$ and $a$. 
To measure the correlations in the prediction space, first we define
\begin{equation}
    \delta_a(x) = O_a(M_q(x)) - O_a(x),
\end{equation}
where $O_a(\cdot)$ is the oracle's prediction of its input for the attribute $a$, $M_q$ is the counterfactual method targeting the query attribute $q$ on an image $x$. 
This measure looks at the signed changes done by $M_q$ on $x$. 
So, now we can measure the relative changes on the attributes when computing a counterfactual example. 
Therefore, we can calculate the correlation coefficient\footnote{The series $\{\delta_a\}_x$ uses solely the successful counterfactual explanations. Further, we used the Pearson Correlation Coefficient to compute $c_{qa}$ and $c_{qa}^{M}$} $c_{qa}^{M}$ between $\{\delta_q(x)\}_x$ and $\{\delta_a(x)\}_x$ to compare it with the true correlation $c_{qa}$. 
Accordingly, we compute the CD as:
\begin{equation}
    CD = \sum_{a} | c_{qa} - c_{qa}^{M} |.
\end{equation}

We apply our proposed metric on DiME and DiVE$^{100}$'s counterfactual explanations. 
We got a CD of 2.30 while DiVE$^{100}$ 2.36 on CelebA's validation set.
With these results, we clearly see that DiME outperform DiVE on the CD metric. 
Nevertheless, the metric shows a difference only by small margin. 
On the one hand, this reveal that DiME and DiVE$^{100}$ have similar capabilities of finding spurious correlations. 
On the other hand, the CD clearly demonstrates that the MNAC results on Table~\ref{tab:main_results} evidence a misleading sense of better performance. 
Although our method has significant margin on the MNAC, DiME outperform DiVE by a small margin on the DC metric.


\subsection{Ablation Studies}\label{sec:ablations}

To assess each component of our proposed pipeline for counterfactual explanations without over-fitting the results over the validation set, we created a small and randomly selected mini-val. 
This subset contains 1,000 images, \textit{i.e.} $\sim$5\% of instances from the validation set of CelebA. 
We focus solely on the category smile for the ablation study.
Quantitatively, we will compute four metrics of interest. 
We used the FID to measure the realism of the explanations, the flip ratio (FR), and the BKL between the target distribution $y$ and counterfactual image distribution to assess the validity and the mean $\ell_1$ loss on the pixel space to evaluate the proximity. 

The BKL metric is the mean of the target label's inverse probability. Thus, we compute it with $BKL(y||C(x)) = 1 - C(y | x)$. 
A low BKL means that the classifier under observation classifies the CEs with high confidence. 
A high BKL means that the CEs are borderline cases where the classifier is not confident of its decision. 
Hence, providing valueless information for inspection. 
Nevertheless, the BKL origin comes from bounding the Kullback-Liebler divergence. 
We will comment more about this metric on the supplementary material.

We computed the FID between all the mini-val instances and the successful counterfactuals. 
Furthermore, due to the different success rates of ablated models, we compute the FID using the least number of examples in the experiment for a fair comparison.
We denote this fair FID as FID$^+$.
Similarly, we compute the $\ell_1$ and BKL solely for successful counterfactuals. 
We proposed these metrics uniquely to assess the validity of the counterfactual explanations. 
Recall that CEs must be close to the input instances. 
Further, to avoid ambiguous CEs, the classifier's prediction for the CEs should be confident. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Integrating the input classifier.} 
In this experiment, we analyze the most essential feature of our pipeline to generate counterfactual explanations. 
On the one hand, remember that traditionally high-stakes applications use standard vision models. 
Further, these models do not perform well on noisy instances due to their exclusive training on clean images. 
On the other hand, the guided diffusion process uses a classifier trained with corrupt data to leverage the gradients on the noisy manifold. 
Therefore, incorporating a clean classifier into our pipeline for CE is a challenge. 
So, we sample a clean image at each time step using the DDPM's unconditional generation to compute the clean gradient to guide the diffusion process. 
To ablate the contribution of the unconditional sampling at each time step, we propose four different methods to use the input classifier in observation. 
The first one, dubbed \emph{Naive}, uses the gradient of the input image at each time step to guide the optimization process. 
The second variation, called \emph{Direct}, uses the noisy instance $z_t$ directly to compute the $\Tilde{L}$ loss instead of $x_t$. 
In this case, we removed the constant $\nicefrac{1}{\sqrt{\alpha_t}}$ since we compute directly the gradients. 
The third ablation sets the CE as the first instance found in the series $\{x_t\}$, \textit{i.e.} $x_t$ with the highest $t$ such that the classifier predicts the target. 
We name this approach \emph{Early Stopping}. 
The last variation uses the DDPM generation without any guiding and beginning from the corrupted image at time-step $\tau$. 
When evaluating the unconditional generation's FID, we use any synthesized image to mark a reference of the performance of the DDPM model.   

\input{tables/naive}

We show the results of this ablation in Table~\ref{tab:naive}. 
Given the low \textit{Direct}'s flip rate, we recompute the unmodified version, the \textit{Naive}, the \emph{Early Stopping}, and the Unconditional FIDs 10 times and report their standard deviation as well on the FID$^+$ column. 
At first glance, we expected the unconditional generation to have lower FID than DiME and the ablated methods. 
Nevertheless, the visual statistics between the query image and the explanation resembles because the perceptual loss further guides the image synthesis into similar images. 
Because the unconditional DDPM does not enjoy from this loss, the generated images have similar coarse attributes but distinct fine-grained details. 
Therefore, the unconditional FID is higher. 
Similarly, the early stopping ablation shows us a similar behaviour. 
Taking the first instance that flips the input's prediction implies a high FR. 
Regardless, many instances found the explanations at an early stage, hence the CEs are ``far'' from the input. 

Secondly, we observe that integrating the clean gradients at each step provides different advantages. 
Our approach has a significant improvement on all metrics. 
The \textit{Direct} method's gradients are useless due to the classifier's inability to predict noisy data. 
We see that the generation quality is proximal to the proposed pipeline, while the FR decreases significantly, telling that most gradients mix with the noise. 
The naive method's gradients are always equal and do not take advantage of the stochasticity process within the DDPM. 
Hence, each time step uses static gradients guiding the diffusion process into a unique direction, independent of the noise. 
%\guillaume{This shows that the stochasticity is necessary to create a valid counterfactual and that using a single instance instead of multiple at each time step is enough, as stated on line 259-262 (?).}
Due to their aggregation at each time step, the final instance presents weird artifacts. 
Lastly, stopping the algorithm early suggests that several instances are borderline cases; henceforth this experiment presents a high BKL.
On the supplementary material, we included visualizations for all ablated models.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \textbf{Gradient Scale.}
% The work Dhariwal and Nichol~\cite{Dhariwal2021DiffusionMB} ablates the scale of the classifier. 
% Their results indicate a positive correlation between the quality of the images, measured with the FID, and the gradients' scale. 
% So, we perform a similar study; to find a counterfactual explanation, we optimize the image formation with three different scales $\lambda_{c} \in \{8, 10, 15\}$ and choose the generated image with the smallest scale. 
% Therefore, we analyze the individual contribution of each scale. 

% We report the results in Table~\ref{tab:gradients}. 
% In our case, we observe the opposite than~\cite{Dhariwal2021DiffusionMB}: when increasing the gradient scale, the FID decreases. 
% The main difference between their ablation and ours is that we begin from an intermediate step while they do not. 
% This subtle difference shows that including gradients on the first iterations of the diffusion process is essential to instantiate the coarse features of the images, \textit{i.e.} the low frequencies of the diffusion process. 
% Yet, at intermediate time steps higher scales disturb the image quality. 

% In our particular context for CEs, we noticed a trade-off between the success rate and the quality of the images. 
% Since we seek to produce sparse modifications, we created most explanations using the lowest scale. 
% Thus, we enjoy the benefits of high-quality images. 
% Further, we boost the FR by using higher scales at the cost of lowering the quality. 
% Adding too much gradient produces outlier noises. 
% The DDPM cannot recognize this noise, and therefore it produces artifacts on the image. 
% However, these artifacts coincide with patterns such that the classifier recognizes them. 

% \input{tables/grads}

% \textbf{Initialization Step.} 
% Following the previous experiment, we seek to find the main variables to produce valid yet sparse CEs. 
% The other variable of interest is the initialization step $\tau$. 
% A higher $\tau$ implies removing more details; hence it needs to perform more image editing. 
% In this experiment, we vary the initialization step to explore the effects of the noise level needed for modifications. 
% We report the results in Table~\ref{tab:steps}. 
% The hyperparameter $\tau$ has a similar effect to the gradient scale $\lambda_c$; we observe a negative correlation between $\tau$ and the FID, and a positive one between $\tau$ and the FR. 
% The image generation has more optimization steps when increasing the initial noise level. 
% Thus, it easily reaches a counterfactual that fools the classifier at the cost of decreasing the CE sparsity, an unwanted effect in the CE community. 
% Similarly, a low $\tau$ increases the sparsity, but the CEs are not as successful. 
% Choosing $\tau=60$ finds an optimal equilibrium between both factors.


% \input{tables/steps}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textbf{Distribution Overtime.} 
% Our pipeline uses the unconditional DDPM to enable the use of the classifier under observation. 
% At each time step, the classifier uses the generated image to compute the gradient with respect to the target label. 
% Therefore, this image gives information on the optimization process at each time step. 
% Hence, in this experiment, we explore the behavior of these images at each stage of the denoising process. 
% To accomplish this, we plot the probability of the target class given by the inspected architecture at each step. 

% In Fig.~\ref{fig:dist_on_time} we visualize the evolution of the target labels' probability over time, along with some examples. 
% We see that the probability increases on time on expectancy. 
% Nevertheless, the example instances show sporadic and non-steady development. 
% Yet, we still observe an ascending behavior. 
% Near the first steps, we see the most unstable conduct. 
% Nonetheless, when reaching a lower number of steps, at $t$ more or less equal to 20, the optimization begins to settle. 
% We attribute this behavior to the decreased invariance along time; when the image generation reaches the final steps, the variance reaches cero. 
% Hence, the unconditional generation does not vary much, reaching an equilibrium.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.90\textwidth]{images/distontime.pdf}
%     \caption{\textbf{Target distribution at each time-step.} We visualize the evolution of the target labels' probability. Each purple line represents a quantile of the probabilities. The color curves are cases shown on the right. In expectancy, the clean image at each time step increases. Nonetheless, typically the curves are sporadic. Yet, we observe an increase.}
%     \label{fig:dist_on_time}
% \end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% comment this if we want to include the gradient and tau experiments.

We further investigate the variables that affect the generation of counterfactual explanations in the supplementary material. 
We included the results of varying the initial noise level $\tau$ and the gradient's scale $\lambda_c$. Furthermore, we included an analysis on the series of clean images produced each time step as well a discussion of the limitations of our algorithm.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Qualitative Results}

We visualize some inputs (left) and the counterfactual examples (right) produced by DiME in Fig.~\ref{fig:qualitative}. 
We show visualizations for the attributes smile and young, yet we will include visualizations for other categories in the supplementary material. 
At first glance, the results reveal that the model performs semantical editings into the input image.
However, uncorrelated features and coarse structure remain almost unaltered. 
We observe small variations on some items, such as the pendants, or out-of-distribution shapes such as hands. 
DiME fails to reconstruct the exact shape of these objects, but the essential aspect remains the same.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.93\textwidth]{images/qualitative.pdf}
    \caption{\textbf{Qualitative Results.} We visualize some images and its corresponding counterfactual explanation produced by our proposed approach. Our methodology achieves to incorporate small but perceptually tangible changes in the image. NS stands for Non-Smiley.}
    \label{fig:qualitative}
    \vspace{-0.4cm}
\end{figure}

% \subsection{Limitations}

% Our pipeline for counterfactual explanation has several limitations. 
% Although we show the benefits of using our model to generate CEs, we are far from accomplishing all aspects crucial for the XAI community. 
% First of all, our method is slow and computationally demanding. 
% Since we are using DDPMs, we adopt most of their limitations. 
% For instance, we need to use the DDPM model $\sim$1800 times to generate a single explanation. 
% This aspect is undesired given that the user requires an explanation on the fly. 
% Finally, we require access to the training data. 
% This limitation is common in many previous studies. 
% However, this aspect is vital in fields where data is sensitive. 
% Although access to the training data is permitted in many cases, we restrict ourselves to using the data without any labels. 


==> sections/temp_method.tex <==
\section{Methodology}

\subsection{Preliminaries}

We begin by introducing the generation process of diffusion models. 
They rely on two Markov chain sampling schemes that are inverse of one another. 
In the forward direction, the sampling starts from a natural image $x$ and iteratively sample $z_1,\cdots,z_T$ by replacing part of the signal with white Gaussian noise. 
More precisely, letting $\beta_t$ be a prescribed variance, the forward process follows the recursive expression:
\begin{equation} \label{eq:degradation_onestep}
    z_t \sim \mathcal{N} (\sqrt{1-\beta_t}\,z_{t-1},  \beta_t \,I),
\end{equation}
where $\mathcal{N}$ is the normal distribution, $I$ the identity matrix, and $z_0 = x$. In fact, this process can be simulated directly from the original sample with 
\begin{equation} \label{eq:degradation}
    z_t \sim \mathcal{N} (\sqrt{\alpha_t}x, (1 - \alpha_t) I),
\end{equation}
where $\alpha_t := \prod_{k=1}^t (1 - \beta_k)$. For clarification, through the rest of the paper, we will refer to clean images with an $x$, while noisy ones with $z$. 


In the reverse process, a neural network progressively denoises $z_T$ to recover the previous samples $z_{T-1},\cdots, z_0$. This network takes the current time step $t$ and a noisy sample $z_t$ as inputs, and produces an average sample $\mu(t, z_t)$ and a covariance matrix $\Sigma(t,z_t)$, shorthanded as $\mu(z_t)$ and $\Sigma(z_t)$, respectively. Then $z_{t-1}$ is sampled with 
\begin{equation} \label{eq:sampling}
    z_{t-1} \sim \mathcal{N}(\mu(z_t), \Sigma(z_t)).
\end{equation}
So, the DDPM algorithm iteratively employs Eq.~\ref{eq:sampling} to generate an image $z_0$ with zero variance, \textit{i.e.} a clean image. Some diffusion models use external information, such as labels, to condition the denoising process. However, in this paper, we employ an unconditional DDPM. 
Hence, apart from the time step $t$, the diffusion model only uses the noisy instance $z_t$ as input.


In practice, the series of variances $\{\beta_t\}$ set $z_T$ such that $z_T\sim \mathcal{N}(0,I)$. Further, the DDPM's trainable parameters are fitted so that the reverse and forward processes share the same distribution.
For details on training schemes, we recommend the studies of Ho \emph{et al.}~\cite{NEURIPS2020_4c5bcfec} and Nichol and Dhariwal~\cite{nichol2021improved} to the reader.
Once the network is trained, one can rely on the reverse Markov chain process to generate a clean image from a random noise image $z_T$. 
Besides, the sampling procedure can be adapted to optimize some properties following the so-called \emph{guided diffusion} scheme proposed in \cite{Dhariwal2021DiffusionMB}\footnote{In \cite{Dhariwal2021DiffusionMB}, the guided diffusion is restricted to a specific classification loss. Still, for the sake of generality and conciseness, we provide its extension to an arbitrary loss}:
\begin{equation} \label{eq:generalized-diff}
    z_{t-1} \sim \mathcal{N}(\mu(z_t) - \Sigma(z_t)\, \nabla_{z_t} L(z_t; y), \Sigma(z_t)),
\end{equation}
where $L$ is a loss function using $z_t$ to specify the wanted property of the generated image, for example, to condition the generation on a prescribed label $y$.

\subsection{DiME: Diffusion Models for Counterfactual Explanations}

We take an image editing standpoint on CE generation, as illustrated Fig.~\ref{fig:baselinecf}. 
We start from a query image $x$. 
Initially, we rely on the forward process starting from $x_\tau=x$ to compute a noisy version $z_\tau$, with $1\leq\tau\leq T$.
Then we go back in the reverse Markov chain using the guided diffusion (Eq~\ref{eq:generalized-diff}) to recover an altered version of the query sample. 
Building upon previous approaches for CEs based on other generative models~\cite{Singla2020Explanation,wachter2018CounterfactualExplanationsOpening,jacob2021steex}, we rely on a loss function composed of two components to steer the diffusion process: a classification loss $L_{class}$, and a perceptual loss $L_{perc}$.
The former guides the image edition into imposing the target label, and the latter drives the optimization in terms of proximity.

\input{figures/main-figure}

In the original implementation of the guided diffusion~\cite{Dhariwal2021DiffusionMB}, a classification loss is computed by applying directly a classifier on the current noisy image $z_t$.
This approach is appropriate if the considered classifier can make robust predictions under noisy observations, \textit{e.g.} it was trained on noisy images.
Such an assumption on the classifier under scrutiny would imply a very strong limitation in the context of counterfactual examples.
We therefore circumvent this obstacle by adapting the guided diffusion mechanism. 
To simplify the notations, let $x_t$ be the clean image produced by the iterative unconditional generation on Eq~\ref{eq:sampling} using as the initial condition $z_t$. 
In fact, this makes $x_t$ a \textit{function} of $z_t$ because we denoise $z_t$ iteratively with the diffusion model $t$ times to obtain $x_t$. 
With these notations, we express our loss as:
\begin{equation}\label{eq:loss-func}
L(z_t;y, x) = \mathbb{E}\left[ \lambda_{c} L_{class}(C(y|x_t)) + \lambda_{p} L_{perc}(x_t, x)\right]:=\mathbb{E}\left[\tilde L(x_t; y, x)\right],
\end{equation}
where $C(y|x_t)$ is the posterior probability of the category $y$ given $x_t$.
Note that an expectation is present due to the stochastic nature of $x_t$. 
In practice, computing the loss gradient would require sampling several realizations of $x_t$ and taking an empirical average. 
We restrict ourselves to a single realization per step $t$ for computational reasons and argue that this is not an issue. 
Indeed, we can partly count on an averaging effect along the time steps to cope with the lack of individual empirical averaging.
Besides, the stochastic nature of our implementation is, in fact, an advantage because it introduces more diversity in the produced CEs, a desirable feature as advocated by \cite{Rodriguez_2021_ICCV}.

Despite this first implementation detail, the dependence of the loss on $x_t$, rather than directly from $z_t$, renders the gradient computation more challenging.
Indeed, formally it would require to apply back-propagation from $x_t$ back to $z_t$: 
\begin{equation} \label{eq:clean-grads-general}
    \nabla_{z_t}L(z_t; y, x) = \left(\frac{Dx_t}{Dz_t}\right)^T\cdot\nabla_{x_t}\tilde L(x_t; y, x).\\
\end{equation}
Unfortunately, this computation requires retaining Jacobian information throughout the entire computation graph, which is very deep when $t$ is close to $\tau$. 
As a result, backpropagation is too memory intensive to be considered an option.
To bypass this concern, we shall rely on the forward sampling process, which operates in a single stage (Eq.~\ref{eq:degradation}).
Using the reparametrization trick~\cite{Kingma2014}, one obtains
\begin{equation}
    z_t = \sqrt{\alpha_t} x_t + \sqrt{1 - \alpha_t} \epsilon, \; \epsilon \sim \mathcal{N}(0, \mathbf{I}).
\end{equation}
Thus, by solving $x_t$ from $z_t$, we can leverage the gradients of the loss function with respect to the noisy input, a consequence of the chain rule. 
Henceforth, the gradients of $L$ with respect to the noisy image become
\begin{equation} \label{eq:clean-grads}
    \nabla_{z_t}L(z_t; y, x) = \frac{1}{\sqrt{\alpha_t}} \nabla_{x_t}\tilde L(x_t; y, x).
\end{equation}
This approximation is possible since the DDPM estimates the reverse Markov chain to fit the forward corruption process. Thereby, both processes are similar.

To sum up, Fig.~\ref{fig:baselinecf} depicts the generation of a counterfactual explanation with our algorithm: DiME.
We start by corrupting the input instance $x=x_\tau$ following Eq.~\ref{eq:degradation} up to the noise level $t=\tau$. 
Then, we iterate the following two stages until $t=0$:
\textit{(i)} First, using the gradients of the previous clean instance $x_{t}$ obtained with unconditional DDPM, we guide the diffusion process to obtain $z_{t-1}$ using Eq.~\ref{eq:generalized-diff} with the gradients computed in Eq.~\ref{eq:clean-grads}. 
\textit{(ii)} Next, we estimate the clean image for the current time step $z_{t-1}$ with the unconditional generation pipeline of DDPMs. 
The final instance is the counterfactual explanation. 
If we do not find an explanation that fools the classifier under observation, we increase the constant $\lambda_c$ and repeat the process.

In the supplemental material we included all implementation details for our method.

% \textbf{Implementation Details.} 
% To train the unconditional DDPM model, we used the publicly available code of~\cite{Dhariwal2021DiffusionMB}. 
% We include all training and architectural details in the supplemental material. 
% In practice, we incorporate additionally an $\ell_1$ loss, $\eta || z_t - x ||_1$, between the noisy image $z_t$ and the input $x$ to improve the $\ell_1$ metric on the pixel space. 
% We empirically set $\eta$ small to avoid any significant impact on the quality of the explanations. 
% Our diffusion model generates faces using 500 diffusion steps from the normal distribution. 
% We re-spaced the sampling process to boost inference speed to generate images with 200 time-steps at test time. 
% We use the following hyper-parameters settings:  $\lambda_{p}=30$, $\eta=0.05$, and $\tau=60$. 
% Finally, we set $\lambda_{c} \in \{8, 10, 15\}$ to iteratively find the counterfactuals. 
% We consider that our method failed if we do not find any explanation after iterating the $\lambda_c$ constants.

==> sections/unused.tex <==
\section{Methodology}

\subsection{Preliminaries}

We begin by introducing the generation process of diffusion models. Let $\mu, \Sigma$ be the mean and covariance matrix models of the DDPM model. The DDPM pipeline to generate an image follows the iterative sampling
\begin{equation} \label{eq:sampling}
    x_{t-1} \sim \mathcal{N}(\mu(x_t), \Sigma(x_t)),
\end{equation}
where $\mathcal{N}$ is the normal distribution, $x_T \sim \mathcal{N}(0, \mathbf{I})$, and $T$ is the total number of steps. Other diffusion models focus on directly extracting the noise $\epsilon$ introduced at each time step \loic{(I don't get that sentence)}. Therefore, it iteratively denoises the initial instance $x_T$ until reaching $x_0$. To optimize the image to produce an image with a target category $y$, Dhariwal \emph{et al.}~\cite{Dhariwal2021DiffusionMB} leverages the log probability gradients with respect to $x_t$, extracted from a classifier $C^N$ trained on noisy images. For simplicity, we will refer to $C^N$ as a \textit{noisy classifier}. Hence, biasing the generation process, mimicking an optimization step:
\begin{equation} \label{eq:guided-diffusion}
    x_{t-1} \sim \mathcal{N}(\mu(x_t) + s \Sigma(x_t) \nabla_{x_t} \log(C^N(y|x_t)), \Sigma(x_t)).
\end{equation}
Here, $s$ is the learning rate and $C^N(y|x_t)$ is the probability of $y$ given its input noisy $x_t$. Accordingly, this formulation resembles a Langevin Dynamics process~\cite{NEURIPS2020_4c5bcfec,song2021denoising,song2021scorebased}. If we generalize the optimization step to follow any loss function $L$, Eq.~\ref{eq:guided-diffusion} becomes
\begin{equation} \label{eq:generalized-diff}
    x_{t-1} \sim \mathcal{N}(\mu(x_t) - \Sigma(x_t) \nabla_{x_t} L(x_t, y), \Sigma(x_t)).
\end{equation}
This iteration step is known as \emph{guided diffusion}.
The optimization terminates when we sample $x_0$.

\loic{I think the next paragraph is not well organised. It gives details that are not essential to understand our approach (apart from clarifying some notations), and it does not help understanding the gist of DDPM training. We need to rework it. Besides, if we want to give some understanding on the principle of DDPM, it would be probably better to do it at the begining of the session.}
The training scheme of these models involves minimizing the variational lower bound between the known posterior probabilities $q(x_{t-1}|x_t, x_0)$ and the DDPM model prediction. For further details on training schemes, we recommend the studies of Ho \emph{et al.}~\cite{NEURIPS2020_4c5bcfec} and Nichol and Dhariwal~\cite{nichol2021improved} to the reader. Given the sequence of variances $\{\beta_i\}_{i=1}^T$, and using the notation $\alpha_i := \prod_{t=1}^i (1 - \beta_t)$, the training of the DDPM becomes simple because we can sample directly $x_t$ from a clean image $\mathtt{I}$ following \loic{I don't like the notation, maybe consider renaming $I$ as $x_0$ (Ok I kept reading, and I understand that you mean to distinguish between noisy and clean images ($x_t$ vs $I_t$).}
\begin{equation} \label{eq:degradation}
    x_t \sim \mathcal{N} (\sqrt{\alpha_t} \mathtt{I}, (1 - \alpha_t) \mathcal{I}).
\end{equation}
where $\mathcal{I}$ is the identity matrix. For the rest of the paper, we will refer to noisy instances with an $x$ while clean instances with an $\mathtt{I}$.

\subsection{Counterfactual Generation}

Eq. \ref{eq:generalized-diff} depicts the inner working of the guided diffusion generation.
So, in order to successfully generate a counterfactual example for an input instance $\mathtt{I}$, we must carefully choose the loss function.
CE methods based on iterative refining steps~\cite{Singla2020Explanation,Wachter2017CounterfactualEW,jacob2021steex} follow a loss function with two components: a classification loss $L_{class}$, and a distance function $L_{dist}$.
The former guides the image generation into predicting the target label, and the latter drives the optimization in terms of proximity.
Hence, the loss function takes the form
\begin{equation}\label{eq:loss-func}
    L(x_t, \mathtt{I}, y) = L_{class}(x_t, y) + L_{dist}(\mathtt{I}, x_t).
\end{equation}
Thus, to generate counterfactual examples, we follow the iterative denoising process from Eq.~\ref{eq:generalized-diff} using the loss function on Eq.~\ref{eq:loss-func}, and instantiating the initial step as a perturbed instance extracted from the degradation process (Eq.~\ref{eq:degradation}) at an intermediate time-step $\tau < T$.

In the guided diffusion pipeline of Dhariwal and Nichol~\cite{Dhariwal2021DiffusionMB}, the classification loss function $L_{class}$ on Eq.~\ref{eq:loss-func} is computed with a noisy classifier, \textit{i.e.} a classifier trained on all levels of noise levels. Nevertheless, in the counterfactual explanations' setup, we are trying to explain a classifier that was trained solely with clean instances. Hence, we cannot use the classifier's gradients directly. To circumvent this concern, we analyze Eq.~\ref{eq:degradation}. By using the reparametrization trick~\cite{Kingma2014}, Eq.~\ref{eq:degradation} becomes
\begin{equation}
    x_t = \sqrt{\alpha_t} \mathtt{I} + \sqrt{1 - \alpha_t} \epsilon, \; \epsilon \sim \mathcal{N}(0, \mathbf{I}).
\end{equation}
Thus, by solving $\mathtt{I}$ from $x_t$, we are able to leverage the gradients of the loss function with respect to the noisy input by using a clean classifier $C$, a consequence of the chain rule. Henceforth, the gradients of $L_{class}$ with respect to the noisy image becomes
\begin{equation} \label{eq:clean-grads}
    \nabla_{x_t}L_{class}(C(\mathtt{I}(x_t)), y) = \frac{1}{\sqrt{\alpha_t}} \nabla_{\mathtt{I}}L_{class}(C(\mathtt{I})), y).
\end{equation}

\input{figures/main-figure}

\textbf{Incorporating a clean classifier.} Eq.~\ref{eq:clean-grads} show us that clean images provide useful information for guiding the model generation. However, we argue that this step only works for the first update step. As Eq.~\ref{eq:degradation} instantiate the initial noisy image $x_\tau$ from the input instance $\mathtt{I}$, the guided diffusion process bias the distribution to sample $x_{\tau - 1}$ with the gradients with respect to the loss function. Thus, we can no longer assume that the next iteration step comes from the original instance $\mathtt{I}$, as we sample it from $\mathcal{N}(\mu(x_\tau) - \Sigma(x_\tau)\nabla_{x_\tau}L, \Sigma(x_\tau))$.


To solve this, assume a general setup where $x_{t+1}$ is sampled following Eq.~\ref{eq:degradation}, and the clean image from which $x_{t+1}$ originates, $\mathtt{I}_{t+1}$, is known. Note that $x_t$ and $\mathtt{I}_t$ belong to the noisy and clean image manifolds, respectively. Accordingly, we compute the clean gradients to generate $x_{t+1}$ following Eq.~\ref{eq:clean-grads}. Now, we sample $x_t$ from Eq.~\ref{eq:generalized-diff} but we don't know the clean instance, $\mathtt{I}_t$, from which it is generated. Hence, we estimate it using the unconditional DDPM generation algorithm. Thus, we can continue the guided process using the gradients of the target $y$ predicted by the classifier with respect to $\mathtt{I}_t$:
\begin{equation}
    \nabla_{x_t}L_{class}(x_t, y) = \frac{1}{\sqrt{\alpha_t}} \nabla_{\mathtt{I}_t}L_{class}(\mathtt{I}_t, y).
\end{equation}
Additionally, as $\mathtt{I}_t$ resides on the image manifold, we can utilize it to use a perceptual loss~\cite{Ledig2017PhotoRealisticSI} to further boost the image generation into a perceptually similar image of $I$. Setting $\lambda$ and $\alpha$ as weights values for the classification and perceptual losses, respectively, the gradients for each iteration step are \loic{(It might be better to change the mixing factor from $\alpha$ to $\lambda$ in order to avoid confusion with $\alpha_t$)}:
\begin{equation} \label{eq:grads}
    \nabla_{x_t} L(x_t, \mathtt{I}, y) = \frac{1}{\sqrt{\alpha_t}} \nabla_{\mathtt{I}_t} \left(\lambda L_{class}(C(\mathtt{I}_t)), y) + \alpha L_{perc}(\mathtt{I}_t, \mathtt{I})\right).
\end{equation}

In this way, as shown in Figure~\ref{fig:baselinecf}, to generate the counterfactual explanations \textit{(i)} we first corrupt the input instance $\mathtt{I}$ following Eq.~\ref{eq:degradation} up to the noise level $t=\tau$. \textit{(ii)} Then, using the gradients of the initial instance, we guide the diffusion process using Eq.~\ref{eq:generalized-diff} with the gradients computed in Eq.~\ref{eq:grads}. \textit{(iii)} Next, we estimate the next iteration clean image with the unconditional generation pipeline of DDPMs. \textit{(iv)} Lastly, we iterate \textit{(ii)} and \textit{(iii)} previously mentioned processes until reaching $t=0$. The final instance is our counterfactual explanation.



==> sections/unused_exp.tex <==
\section{Experiments}

\subsection{Implementation Details}

To train the unconditional DDPM model, we used the publicly available code of~\cite{Dhariwal2021DiffusionMB}. 
We include all training and architectural details in the supplemental material. 
In practice, we incorporate additionally an $\ell_1$ loss, $\eta || z_t - x ||_1$, between the noisy image $z_t$ and the input $x$ to improve the $\ell_1$ metric on the pixel space. 
The scalar $\eta$ is its scale value. 
We empirically set $\eta$ small to avoid any significant impact on the quality of the explanations. 
Our diffusion model generates faces using 500 diffusion steps from the normal distribution. 
We re-spaced the sampling process to boost inference speed to generate images with 200 time-steps at test time. 
To find all constants, we explored the hyperspace of parameters optimizing the image quality visually, the flip ratio, the $\ell_1$ norm on the pixel space, and a bounded Kullback-Leibler (BKL) metric on a 1,000 image subset of the validation. 
We will give more details about these metrics and the subset in section~\ref{sec:ablations}. 
We set the scale values as $\lambda_{p}=30$, $\eta=0.05$, and $\tau=60$. 
Finally, we set $\lambda_{c} \in \{8, 10, 15\}$ to iteratively find the counterfactuals. 
We consider that our method failed if we do not find any explanation after iterating the $\lambda_c$ constants.
%\guillaume{Read the final 2 lines of the methodology section to comprehend why I set $\lambda_{c} \in \{8, 10, 15\}$.}


\subsection{Quantitative Validation}

We follow previous works~\cite{Rodriguez_2021_ICCV,Singla2020ExplanationBP} to validate our method for counterfactual explanations.
We study the CelebA dataset~\cite{liu2015faceattributes}, preprocessing all images with a $128\times128$ resolution.
CelebA contains 200k images, labeled with 40 binary attributes.
Previous works validate their methods on the \emph{smile} and \emph{young} binary attributes, ignoring all other features. 
The architecture to explain is a DesNet121~\cite{Huang_2017_CVPR}. 
Quantitatively, we computed three metrics to assess all CEs: Frechet Inception Distance~\cite{NIPS2017_8a1d6947} (FID), Face Verification Accuracy~\cite{8373813} (FVA), and Mean Number of Attributes Changed (MNAC)~\cite{Rodriguez_2021_ICCV}. 
With our hyperparameter selection, we achieved a success rate of 97.6 and 98.9 for the smile and young attributes, respectively.

For the CE community, these metrics evaluate the core aspects of the explanations.
The FID looks at the realism of the explanations. 
This metric informs a general view of the generated counterfactuals' quality. 
Further, the image synthesis adopted this metric as the standard assessment for reality. 
The MNAC and FVA complement each other. 
On the one hand, the MNAC metric looks at the face attributes that changed between the input image and its counterfactual explanation, regarding if the individual's identity changed. 
On the other hand, the FVA looks at the individual's identity without considering the difference of attributes. 
Optimizing these metrics in parallel improves the proximity and sparsity of counterfactual examples, two properties desired for an explanation. 
Rodriguez \textit{et al.}~\cite{Rodriguez_2021_ICCV} do not report a metric for diversity. 
So, in section~\ref{sec:ablations} we included an experiment for diversity to compare ourselves.

\input{tables/main-results}

Given the binary nature of the task, the target label is always the opposite of the prediction. 
If the model correctly estimates an instance's label, we flip the model's forecast. 
Else, we modify the input image to classify the image correctly. 
Additionally, to compute the FID, the FVA, and the MNAC, we consider only those successful counterfactual examples, following previous studies~\cite{Rodriguez_2021_ICCV,Singla2020ExplanationBP}.
To compute the FVA, we used the cosine similarity between the input image and its produced counterfactual on the feature space of a ResNet50~\cite{He2016DeepRL} pretrained model on VGGFace2~\cite{8373813}.
The instance and the explanation share the same identity if the similarity is higher than 0.5.
The mean of these values is the FVA.
To compute the MNAC, we fine-tuned the VGGFace2 model on the CelebA dataset.
We refer to the fine-tuned model as the oracle.
Thus, the MNAC is the mean number of the changed attributes.
Finally, for a fair comparison with previous State-of-the-Art, we trained all classifiers, including the fine-tuned ResNet50 for the MNAC assessment, using the DiVE's~\cite{Rodriguez_2021_ICCV} available code.

DiVE do not report their success rate. 
This rises the concern of the fairness to compare our methods. 
Since the metrics are highly dependant on the number of samples, especially the FID, we recomputed their CEs. 
To our surprise, their flip ratio was quite low (44.6$\%$ for the smile category). 
Therefore, we regenerated the counterfactual explanations with 100 optimization steps and reported the results as DiVE$^{100}$. 
Their success rate is $92.0\%$ and $93.4\%$, which is more comparable to ours. 
We show DiME's performance in Table~\ref{tab:main_results}. 
Our method beats the previous literature in five out of six metrics. 
For instance, we have a $\sim$10 fold improvement on the FID metric for the smile category, while the young attribute has an $\sim$8 fold improvement. 
We credit these gains to the generative capabilities of the diffusion model. 
Further, our generation process does not require entirely corrupting the input instance; hence the coarse details of the image remain. 
The other methods use latent space-based architectures. 
Thus, they require to compact essential information removing outlier data. 
Consequently, the generated CEs cannot reconstruct the missing information, losing significant components of the image statistics. 
Regarding DiVE$^{100}$ results, the over-optimization clearly destroys most aspects that make a person's identity and its attributes. 


%\guillaume{Talk about the DiVE's unknown flip rate, our estimation with their code and the how this affects their performance, specially on the FID metric. Say that our flip rate is 97.6 for smile and 98.9 for young.}

%\guillaume{At the eye of the inception network, the background might contain important information. Removing it produces an increase in the FID metric.}

\guillaume{I do not feel confident with this paragraph}

For the smile category, the input's gradients are localized. 
So, the gradients do not corrupt essential regions in the guided denoising process, enabling our model to perform better in the FVA metric. 
For the other methods, small changes in the image require significant modifications due to the bottleneck. 
In contrast, editing notable features for the face is harder for our model. 
The young feature must change the general appearance of the face. 
Hence, the gradients of the classifier are not sparse. 
Therefore, the gradients might steer the diffusion process in an unwanted direction. 
As a result, many small but essential details change, resulting in a face identity swap.

\subsection{Discovering Spurious Correlations}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/correlations-top10.pdf}
    \caption{\textbf{Spurious Correlation Detection.} We show the top 9 correlated attributes when targeting the smile attribute and the Pearson Correlation Coefficient in absolute value from the ground truth on the training set. Even when the classifier and the oracle have distinct learned biases, both models obey similar behaviors. Hence, DiME is able to detect spurious correlations.}
    \label{fig:correlation}
\end{figure}

The end goal of counterfactual examples is to uncover the modes of error of a target model. 
One way to reveal these susceptibilities is to search for correlations on the changed attributes. 
We might infer a high correlation between the target attribute and other features if there is a pattern on which traits differ. 
Thus, in Figure~\ref{fig:correlation} we exhibit the absolute value of the Pearson Correlation Coefficient between the smile category and the other attributes on the label space in the training set. 
Here, we only show the top 9 most correlated attributes, but we added the missing traits in the supplementary material.

We included the attributes that changed according to the input classifier and the oracle, along with the correlation coefficients. 
Even when these models have different learned biases due to the dataset where each one was trained, both models expose explicit tendencies. 
For instance, we see a clear correlation between the ``High Cheekbones'' and ``Mouth Slightly Open'' attributes. 
Our method enables us to expose clear tendencies in the label space. 
Nevertheless, we see no significant connection between uncorrelated traits.



% PE~\cite{Singla2020Explanation} proposes to evaluate bias detection by looking at an entangled classifier between the smile and male categories, \emph{i.e.} the classifier is trained with all men smiling and all women non-smiling. We argue that this setup is an extreme case of entanglement. Thus, we extend this experiment by entangling the untangled classifier directly. For this experiment, we take the same categories as PE~\cite{Singla2020Explanation}, given that their label correlation is low. In practice, we incorporate a mixing simple factor $0 \leq \phi \leq 1$ between the logits of the chosen categories, $l_{male}$ and $l_{smile}$, as follows:
% \begin{equation}
%     l = \phi \, l_{male} + (1 - \phi) \, l_{smile}.
% \end{equation}
% We explored $\phi \in \{0.0, 0,1, 0.2, 0.3, 0.4, 0.5\}$ and show the changed attributes according to the oracle on Figure~\ref{fig:entangled} for our method and DiVE. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\textwidth]{images/entanglement.pdf}
%     \caption{\textbf{Entanglement.}}
%     \label{fig:entangled}
% \end{figure}





\subsection{Ablation Studies}\label{sec:ablations}

To assess each component of our proposed pipeline for counterfactual explanations without over-fitting the results over the validation set, we created a small and randomly selected mini-val. 
This subset contains 1,000 images, \textit{i.e.} $\sim$5\% of instances from the validation set of CelebA. 
We focus solely on the category smile for the ablation study.
Quantitatively, we will compute four metrics of interest. 
We used the FID to measure the realism of the explanations, the flip ratio (FR), and the BKL between the target distribution $y$ and counterfactual image distribution to assess the validity and the mean $\ell_1$ loss on the pixel space to evaluate the proximity. 

We computed the FID between all the mini-val instances and the successful counterfactuals. 
Furthermore, due to the different success rates of ablated models, we compute the FID using the least number of examples in the experiment for a fair comparison.
We denote this fair FID as FID$^+$.
Similarly, we compute the $\ell_1$ and BKL solely for successful counterfactuals. 
We proposed these metrics uniquely to assess the validity of the counterfactual explanations. 
Recall that CEs must be close to the input instances. 
Further, to avoid ambiguous CEs, the classifier's prediction for the CEs should be confident. 
So, the BKL metric is the mean of the target label's inverse probability: $BKL(y||C(x)) = 1 - C(y | x)$. 
A low BKL means that the classifier under observation classifies the CEs with high confidence. 
A high BKL means that the CEs are borderline cases where the classifier is not confident of its decision. 
Hence, providing valueless information for inspection. 
Nevertheless, the BKL origin comes from bounding the Kullback-Liebler divergence. 
We will comment more about this metric on the supplementary material.


% The Kullback-Liebler divergence has no upper limit. A simple trick to bound its values is to use a bounded non-linearity. Thus, we used the following function to limit the KL divergence:
% \begin{equation}
%     BKL(y||C(x)) = 1 - e^{-KL(y||C(x))}.
% \end{equation}
% The BKL is 0 when the distributions $y$ and $C(x)$ match, and it is 1 when $y$ is the complement of $C(x)$. 
% Due to the target distribution is a one hot vector, the BKL metric becomes:
% \begin{equation}
%     BKL(y||C(x)) = 1 - C(y | x).
% \end{equation}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.83\textwidth]{images/diversity.pdf}
    \caption{\textbf{Diversity Counterfactual examples.} The classifier predicts first two input images as non-smiley and the last two as smiley. Our CE pipeline is capable of synthesising divers counterfactual without any explicit mechanism.}
    \label{fig:diversity}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Counterfactual Diversity.} 
One of the most crucial traits of counterfactual explanations methodologies is the ability to create multiple and diverse examples~\cite{Rodriguez_2021_ICCV}. 
Creating multiple instances may expose the network's brittleness towards spurious correlations. 
As stated in the methodology section, the DiME's stochastic properties enable the sampling of diverse counterfactuals. 
To measure our method's capabilities to produce multiple explanations, we computed the pair-wise LPIPS~\cite{Zhang_2018_CVPR_Unreasonable} metric between 5 independent runs varying the initial seed. 
We want to compute the dissimilarities between the counterfactuals, so we exclude the input instance to compute the metric. 
A higher LPIPS means increased perceptual dissimilarities between the explanations, hence, more diversity. 
We compare our results with DiVE and its Fisher Spectral variant. 
Both versions produce eight counterfactual explanations simultaneously and have an explicit mechanism to create different images. 

Our experimentation with DiVE shows that their success rate is relatively low. 
Hence, we set their optimization iterations to 100 to reach a similar FR. 
Even with this fine-tuned hyperparameter, DiVE Fisher Spectral's FR is substantially worst and does not achieve comparable success rates. 
We visualize some examples in Fig.~\ref{fig:diversity} and show the performance of the five runs on the supplementary material. 
We obtained an LPIPS value of 0.213. 
In contrast, DiVE~\cite{Rodriguez_2021_ICCV} and its Spectral Fisher variant obtained an LPIPS of 0.044 and 0.086, respectively. 
Recall that DiME does not have an explicit mechanism to create diverse counterfactuals. 
Its only mechanism is the stochasticity within the sampling process, refer to Eqs.~\ref{eq:sampling} and~\ref{eq:generalized-diff}.
In contrast, DiVE has a diversity loss when optimizing the eight explanations. 
Yet, our methodology achieves higher diversity with the LPIPS metric even without an explicit mechanism. 

\guillaume{I think this should be first than the variability experiment. For me is more important. What do you think?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Integrating the input classifier.} 
In this experiment, we analyze the most essential feature of our pipeline to generate counterfactual explanations. 
On the one hand, remember that traditionally high-stakes applications use standard vision models. 
Further, these models do not perform well on noisy instances due to their exclusive training on clean images. 
On the other hand, the guided diffusion process uses a classifier trained with corrupt data to leverage the gradients on the noisy manifold. 
Therefore, incorporating a clean classifier into our pipeline for CE is a challenge. 
So, we sample a clean image at each time step using the DDPM's unconditional generation to compute the clean gradient to guide the diffusion process. 
To ablate the contribution of the unconditional sampling at each time step, we propose four different methods to use the input classifier in observation. 
The first one, dubbed \emph{Naive}, uses the gradient of the input image at each time step to guide the optimization process. 
The second variation, called \emph{Direct}, uses the noisy instance $z_t$ directly to compute the $\Tilde{L}$ loss instead of $x_t$. 
In this case, we removed the constant $\nicefrac{1}{\sqrt{\alpha_t}}$ since we compute directly the gradients. 
The third ablation sets the CE as the first instance found in the series $\{x_t\}$, \textit{i.e.} $x_t$ with the highest $t$ such that the classifier predicts the target. 
We name this approach \emph{Early Stopping}. 
The last variation uses the DDPM generation without any guiding and beginning from the corrupted image at time-step $\tau$. 
When evaluating the unconditional generation's FID, we use any synthesized image to mark a reference of the performance of the DDPM model.   

\input{tables/naive}

We show the results of this ablation in Table~\ref{tab:naive}. 
Given the low \textit{Direct}'s flip rate, we recompute the unmodified version, the \textit{Naive}, the \emph{Early Stopping}, and the Unconditional FIDs 10 times and report their standard deviation as well on the FID$^+$ column. 
At first glance, we expected the unconditional generation to have lower FID than DiME and the ablated methods. 
Nevertheless, the visual statistics between the query image and the explanation resembles because the perceptual loss further guides the image synthesis into similar images. 
Because the unconditional DDPM does not enjoy from this loss, the generated images have similar coarse attributes but distinct fine-grained details. 
Therefore, the unconditional FID is higher. 
Similarly, the early stopping ablation shows us a similar behaviour. 
Taking the first instance that flips the input's prediction implies a high FR. 
Regardless, many instances found the explanations at an early stage, hence the CEs are ``far'' from the input. 

Secondly, we observe that integrating the clean gradients at each step provides different advantages. 
Our approach has a significant improvement on all metrics. 
The \textit{Direct} method's gradients are useless due to the classifier's inability to predict noisy data. 
We see that the generation quality is proximal to the proposed pipeline, while the FR decreases significantly, telling that most gradients mix with the noise. 
The naive method's gradients are always equal and do not take advantage of the stochasticity process within the DDPM. 
Hence, each time step uses static gradients guiding the diffusion process into a unique direction, independent of the noise. 
%\guillaume{This shows that the stochasticity is necessary to create a valid counterfactual and that using a single instance instead of multiple at each time step is enough, as stated on line 259-262 (?).}
Due to their aggregation at each time step, the final instance presents weird artifacts. 
Lastly, stopping the algorithm early suggests that several instances are borderline cases; henceforth this experiment presents a high BKL.
On the supplementary material, we included visualizations for all ablated models.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\textbf{Gradient Scale.}
The work Dhariwal and Nichol~\cite{Dhariwal2021DiffusionMB} ablates the scale of the classifier. 
Their results indicate a positive correlation between the quality of the images, measured with the FID, and the gradients' scale. 
So, we perform a similar study; to find a counterfactual explanation, we optimize the image formation with three different scales $\lambda_{c} \in \{8, 10, 15\}$ and choose the generated image with the smallest scale. 
Therefore, we analyze the individual contribution of each scale. 

We report the results in Table~\ref{tab:gradients}. 
In our case, we observe the opposite than~\cite{Dhariwal2021DiffusionMB}: when increasing the gradient scale, the FID decreases. 
The main difference between their ablation and ours is that we begin from an intermediate step while they do not. 
This subtle difference shows that including gradients on the first iterations of the diffusion process is essential to instantiate the coarse features of the images, \textit{i.e.} the low frequencies of the diffusion process. 
Yet, higher scales at intermediate time steps disturb the image quality. 

In our particular context for CEs, we noticed a trade-off between the success rate and the quality of the images. 
Since we seek to produce sparse modifications, we created most explanations using the lowest scale. 
Thus, we enjoy the benefits of high-quality images. 
Further, we boost the FR by using higher scales at the cost of lowering the quality. 
Adding too much gradient produces outlier noises. 
The DDPM cannot recognize this noise, and therefore it produces artifacts on the image. 
However, these artifacts coincide with patterns such that the classifier recognizes them. 

\input{tables/grads}

\textbf{Initialization Step.} 
Following the previous experiment, we seek to find the main variables to produce valid yet sparse CEs. 
The other variable of interest is the initialization step $\tau$. 
A higher $\tau$ implies removing more details; hence it needs to perform more image editing. 
In this experiment, we vary the initialization step to explore the effects of the noise level needed for modifications. 
We report the results in Table~\ref{tab:steps}. 
The hyperparameter $\tau$ has a similar effect to the gradient scale $\lambda_c$; we observe a negative correlation between $\tau$ and the FID, and a positive one between $\tau$ and the FR. 
The image generation has more optimization steps when increasing the initial noise level. 
Thus, it easily reaches a counterfactual that fools the classifier at the cost of decreasing the CE sparsity, unwanted effect in the CE community. 
Similarly, a low $\tau$ increases the sparsity, but the CEs are not as successful. 
Choosing $\tau=60$ finds an optimal equilibrium between both factors.


\input{tables/steps}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Distribution Overtime.} 
Our pipeline uses the unconditional DDPM to enable the use of the classifier under observation. 
At each time step, the classifier uses the generated image to compute the gradient with respect to the target label. 
Therefore, this image gives information on the optimization process at each time step. 
Hence, in this experiment, we explore the behavior of these images at each stage of the denoising process. 
To accomplish this, we plot the probability of the target class given by the inspected architecture at each step. 

In Fig.~\ref{fig:dist_on_time} we visualize the evolution of the target labels' probability over time, along with some examples. 
We see that the probability increases on time on expectancy. 
Nevertheless, the example instances show sporadic and non-steady development. 
Yet, we still observe an ascending behavior. 
Near the first steps, we see the most unstable conduct. 
Nonetheless, when reaching a lower number of steps, at $t$ more or less equal to 20, the optimization begins to settle. 
We attribute this behavior to the decreased invariance along time; when the image generation reaches the final steps, the variance reaches cero. 
Hence, the unconditional generation does not vary much, reaching an equilibrium.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.90\textwidth]{images/distontime.pdf}
    \caption{\textbf{Target distribution at each time-step.} We visualize the evolution of the target labels' probability. Each purple line represents a quantile of the probabilities. The color curves are cases shown on the right. In expectancy, the clean image at each time step increases. Nonetheless, typically the curves are sporadic. Yet, we observe an increase.}
    \label{fig:dist_on_time}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% comment this if we want to include the gradient and tau experiments.

% We further investigate the variables that affect the generation of counterfactual explanations in the supplementary material. 
% We included the results of varying the initial noise level $\tau$ and the gradient's scale $\lambda_c$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Qualitative Results}

We visualize some inputs (left) and the counterfactual examples (right) produced by DiME in Fig.~\ref{fig:qualitative}. 
We show visualizations for the attributes smile and young, yet we will include visualizations for other categories in the supplementary material. 
At first glance, the results reveal that the model performs semantical editings into the input image.
However, uncorrelated features and coarse structure remain almost unaltered. 
We observe small variations on some items, such as the pendants, or out-of-distribution shapes such as hands. 
DiME fails to reconstruct the exact shape of these objects, but the essential aspect remains the same.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.93\textwidth]{images/qualitative.pdf}
    \caption{\textbf{Qualitative Results.} We visualize some images and its corresponding counterfactual explanation produced by our proposed approach. Our methodology achieves to incorporate small but perceptually tangible changes in the image. NS stands for Non-Smiley.}
    \label{fig:qualitative}
\end{figure}

\subsection{Limitations}

Our pipeline for counterfactual explanation has several limitations. 
Although we show the benefits of using our model to generate CEs, we are far from accomplishing all aspects crucial for the XAI community. 
First of all, our method is slow and computationally demanding. 
Since we are using DDPMs, we adopt most of their limitations. 
For instance, we need to use the DDPM model $\sim$1800 times to generate a single explanation. 
This aspect is undesired given that the user requires an explanation on the fly. 
Finally, we require access to the training data. 
This limitation is common in many previous studies. 
However, this aspect is vital in fields where data is sensitive. 
Although access to the training data is permitted in many cases, we restrict ourselves to using the data without any labels. 

